Nonexistence of Wandering Domains for Infinitely Renormalizable H\'enon Maps

This article extends the theorem of the absence of wandering domains from unimodal maps to infinitely period-doubling renormalizable H\'enon-like maps in the strongly dissipative (area contracting) regime. The theorem solves an open problem proposed by several authors [van Strien (2010) and Lyubich and Martens (2011)], and covers a class of maps in the nonhyperbolic higher dimensional setting. The classical proof for unimodal maps breaks down in the H\'enon settings, and two techniques, "the area argument" and "the good region and the bad region", are introduced to resolve the main difficulty. The theorem also helps to understand the topological structure of the heteroclinic web for such kind of maps: the union of the stable manifolds for all periodic points is dense.

==> Graph_pullback_lemma.tex <==
\begin{lemma}
\label{lem:Graph pullback}Given $m>0$, $\delta>0$, $\overline{\epsilon}>0$,
$I\subset I^{h}\subset I^{v}$, and $F\in\mathcal{H}_{\delta}(I^{h}\times I^{v},\overline{\epsilon})$.
Assume that $U,U'\subset I^{h}$ are two closed intervals such that
$F(x,y)=(h_{y}(x),x)$ satisfies the properties for all $y\in I^{v}$
\begin{enumerate}
\item $h_{y}(U')\supset U$ and 
\item $\left\Vert h_{y}'\right\Vert _{U'}=\sup_{x\in U'}\left|\frac{\partial h}{\partial x}(x,y)\right|\geq m$.
\end{enumerate}
If $\Gamma\subset U\times I^{h}$ is the vertical graph of some $L$-Lipschitz
function on $I^{h}$ with $L<m$, then the preimage $F^{-1}(\Gamma)\cap U'\times I^{v}$
is the vertical graph of some $\frac{1}{\delta(m-L)}\left\Vert \epsilon\right\Vert $-Lipschitz
function on $I^{v}$.
\end{lemma}
\begin{proof}
Assume that $\Gamma$ is the vertical graph of a $L$-Lipschitz function
$\gamma:I^{h}\rightarrow U$.

First, we prove that $F^{-1}(\Gamma)\cap U'\times I^{v}$ is a vertical
graph of some function on $I^{v}$. Fixed $y\in I^{v}$. Our goal
is to find a unique solution $\hat{\gamma}(y)\in U'$ such that 
\[
F(\hat{\gamma}(y),y)=(h_{y}(\hat{\gamma}(y)),\hat{\gamma}(y))=(\gamma(\hat{\gamma}(y)),\hat{\gamma}(y)),
\]
i.e. the fixed point of $h_{y}^{-1}\circ\gamma$.

By the second condition, $h_{y}$ is injective on $U'$. So the inverse
$h_{y}^{-1}:U\rightarrow U'$ exists. Define $T:U'\subset I^{h}\rightarrow U'$
by $T=h_{y}^{-1}\circ\gamma$. For all $x_{1},x_{2}\in U'$, we have
\begin{eqnarray*}
\left|T(x_{2})-T(x_{1})\right| & = & \left|h_{y}^{-1}\circ\gamma(x_{2})-h_{y}^{-1}\circ\gamma(x_{1})\right|\\
 & \leq & \frac{1}{m}\left|\gamma(x_{2})-\gamma(x_{1})\right|\\
 & \leq & \frac{L}{m}\left|x_{2}-x_{1}\right|.
\end{eqnarray*}
Thus, $T$ is a strong contraction since $L<m$. By the contraction
mapping principle \cite[Theorem 5.7.1]{marsden1993elementary}, $T$
has a unique fixed point $\hat{\gamma}(y)\in U'$. Consequently, $F^{-1}(\Gamma)\cap U'\times I^{v}$
is the vertical graph of $\hat{\gamma}:I^{v}\rightarrow U'$.

It remains to prove that $\hat{\gamma}$ is Lipschitz. Let $y_{1},y_{2}\in I^{v}$
and $x_{i}=\hat{\gamma}(y_{i})$ for $i=1,2$. Then $h_{y_{i}}(x_{i})=\gamma(x_{i})$
for $i=1,2$. We get
\[
\left(h_{y_{2}}(x_{2})-h_{y_{2}}(x_{1})\right)-\left(\gamma(x_{2})-\gamma(x_{1})\right)=h_{y_{1}}(x_{1})-h_{y_{2}}(x_{1}).
\]
For the left hand side of the equality, we have
\begin{eqnarray*}
\left|\left(h_{y_{2}}(x_{2})-h_{y_{2}}(x_{1})\right)-\left(\gamma(x_{2})-\gamma(x_{1})\right)\right| & \geq & \left|h_{y_{2}}(x_{2})-h_{y_{2}}(x_{1})\right|-\left|\gamma(x_{2})-\gamma(x_{1})\right|\\
 & \geq & \left(m-L\right)\left|x_{2}-x_{1}\right|.
\end{eqnarray*}
For the right hand side of the inequality, we have
\[
\left|h_{y_{1}}(x_{1})-h_{y_{2}}(x_{1})\right|\leq\left\Vert \frac{\partial\epsilon}{\partial y}\right\Vert _{I^{h}\times I^{v}}\left|y_{2}-y_{1}\right|\leq\frac{1}{\delta}\left\Vert \epsilon\right\Vert \left|y_{2}-y_{1}\right|.
\]
Combine the two inequalities, we obtain
\[
\left|\hat{\gamma}(y_{2})-\hat{\gamma}(y_{1})\right|\leq\frac{1}{\delta(m-L)}\left\Vert \epsilon\right\Vert \left|y_{2}-y_{1}\right|.
\]
Therefore, $\hat{\gamma}$ is $\frac{1}{\delta(m-L)}$-Lipschitz.
\end{proof}



